Nested Hierarchical Dirichlet Processes for Multi-Level Non-Parametric Admixture Modeling

Dirichlet Process(DP) is a Bayesian non-parametric prior for infinite mixture modeling, where the number of mixture components grows with the number of data items. The Hierarchical Dirichlet Process (HDP), is an extension of DP for grouped data, often used for non-parametric topic modeling, where each group is a mixture over shared mixture densities. The Nested Dirichlet Process (nDP), on the other hand, is an extension of the DP for learning group level distributions from data, simultaneously clustering the groups. It allows group level distributions to be shared across groups in a non-parametric setting, leading to a non-parametric mixture of mixtures. The nCRF extends the nDP for multilevel non-parametric mixture modeling, enabling modeling topic hierarchies. However, the nDP and nCRF do not allow sharing of distributions as required in many applications, motivating the need for multi-level non-parametric admixture modeling. We address this gap by proposing multi-level nested HDPs (nHDP) where the base distribution of the HDP is itself a HDP at each level thereby leading to admixtures of admixtures at each level. Because of couplings between various HDP levels, scaling up is naturally a challenge during inference. We propose a multi-level nested Chinese Restaurant Franchise (nCRF) representation for the nested HDP, with which we outline an inference algorithm based on Gibbs Sampling. We evaluate our model with the two level nHDP for non-parametric entity topic modeling where an inner HDP creates a countably infinite set of topic mixtures and associates them with author entities, while an outer HDP associates documents with these author entities. In our experiments on two real world research corpora, the nHDP is able to generalize significantly better than existing models and detect missing author entities with a reasonable level of accuracy.

==> MultiAuthorModel.tex <==
%\subsection{Nested HDP for Multi-Entity Documents}	
\vspace{0.05in}
\noindent
{\bf Nested HDP for Multi-Entity Documents: }	
The DP-HDP model above associates a single distribution over topics $G'_j$ with the $j$th document, and the topic $\theta_{ji}$ for each word $x_{ji}$ in the document is drawn from $G'_j$.
In the context of entity-topic analysis, this means that a single entity is associated with a document, and words are drawn from the preferred topics of this entity.
However, many applications, such as analyzing entities from news articles and authors from scientific literature, require associating multiple entities with each document, and each word in the document is drawn from a preferred topic of one of these entities.
In this section, we extend the earlier model for multi-entity documents.

%We extend the approach presented in \S~\ref{single} to the setting of multiple entities per document. In the single entity model, since a document is associated with one entity, a single entity is sampled for all the words in the document. Now, in the case of multiple entities per document, first we sample an entity for each word in the document, and then a topic is sampled according to the entity specific distribution of topics. 


As before, we first create a set of distributions $\{G_{k'}\}_{k'=1}^\infty$ over the same set of (topic) distributions $\{\phi_{k}\}_{k=1}^\infty$ ($\phi_k\sim H$) by drawing independently from an HDP, 
%\begin{equation}
%G_{k'}\sim HDP(\{\alpha_{k'}\},\gamma,H)
%\end{equation}
and create a global mixture over them:
\begin{eqnarray*}
G_{k'}\sim HDP(\{\alpha_{k'}\},\gamma,H); &\ \ \  \beta' \sim GEM(\gamma'); & G'_0 \equiv \sum_{k'=1}^\infty \beta'_{k'}\delta_{G_{k'}}
\end{eqnarray*}
This may be interpreted as creating a countable set of entities by defining topic preferences (distributions over topics) for each of them, and then defining a `global popularity' of the entities.
Earlier, for single entity documents, the lone entity was sampled from this global popularity.
Now, we define a document-specific local popularity for entities, derived from this global popularity:
%This is defined as 
\begin{equation}
\label{eqn:ndpLocalPopularity}
G'_j \equiv \sum_{k'=1}^{\infty} \pi'_{jk'}\delta_{G_{k'}},\ \{\pi'_{jk'}\}\sim DP(\alpha'_j,\beta')
\end{equation}
Now, sampling each factor $\theta_{ji}$ in document $j$ is preceded by choosing an entity $\theta'_{ji}\sim G'_j$ by sampling according to local entity popularity.
Note that $P(\theta'_{ji}=G_{k'})=\pi'_{jk'}$. 

Using the stick breaking definition of the HDP in Eqn. \ref{gJstick}, we can see that $G'_j$ is drawn from a HDP.
The base distribution of that HDP has to be the distribution from which the atoms $\{G_{k'}\}$ are drawn, which is again an HDP.
Therefore, we can write:
\begin{equation}
\label{eqn:ndp}
\theta'_{ji} \sim G'_j \sim \mbox{HDP}(\{\alpha'_j\},\gamma',\mbox{HDP}(\{\alpha_{k'}\},\gamma,H))
\end{equation}
We refer to the two relevant HDPs as the inner and outer HDPs. 
Observing the parallel with the nDP definition in Eqn. \ref{eqn:ndp:dpfamily}, we call this the nested HDP (nHDP), and write $\theta'_{ji} \sim  nHDP(\{\alpha'_j\}, \gamma', \{\alpha_{k'}\}, \gamma, H)$.
Similar to the nDP, and the DP-HDP (Eqn. \ref{gJd}), this again defines a distribution over the space of distributions over distributions.
The complete nHDP mixture model is defined by subsequently sampling $\theta_{ji} \sim \theta'_{ji}$, followed by $x_{ji} \sim F(\theta_{ji})$.


%Therefore, in this setting, $G'_{j'}$ is defined as follows
%$$G'_{j'}|\alpha'_{j'}, G'_0  \sim \textnormal{DP}(\alpha'_{j'}, G'_0) \textnormal{~~for each } j',$$
%where $G'_0$ is defined in (\ref{gS}). 

%We can rewrite the above process as HDP$(\bm\alpha', \gamma', \text{HDP}(\bm\alpha,\gamma, H))$ where
%$$G'_{j'}|\alpha'_{j'},\gamma',\bm\alpha,\gamma,H 
%\sim \textnormal{HDP}(\alpha'_{j'},\gamma', \textnormal{HDP}(\bm\alpha, \gamma, H)) ~~~ \text{for each } j'$$
%and therefore, we refer to it as \textit{nested hierarchical Dirichlet process}. 
%The nested HDP process can be used as the prior distribution over the factors  for grouped data. For each group $j'$ let  where a factor $\theta'_{j'i'}$  correspond to the observation $x_{j'i'}$. 

%The above process augmented with \ref{eq:DP-HDPmm} gives us \textit{nested hierarchical Dirichlet process mixture model}.
%\subsubsection{The stick-breaking construction}
%Given that, for each $j'$, $G'_{j'}$ is distributed as a Dirichlet process, it can be expressed using stick-breaking construction
%$$G'_{j'} = \sum_{j=1}^\infty \pi'_{j'j} \delta_{G_j}, $$
%where $ \pi'_{j'} = (\pi'_{j'j})_{j=1}^\infty \sim $ DP$(\alpha'_{j'}, \bm\beta')$ and $(G_j)_{j=1}^{\infty} \stackrel{iid}{\sim}$ HDP$(\alpha_j, \gamma, H)$ as defined in (\ref{gJstick}). 

%For each $j'$, as each $\theta'_{j'i'}$ factor corresponding to  observation $x_{j'i'}$ is distributed according to $G'_{j'}$, it takes value $G_j$ with probability $\pi'_{j'j}$. 
An alternative characterization of the nHDP mixture model is using the topic index $z_{ji}$ and entity index $z'_{ji}$ corresponding to $x_{ji}$:
%We obtain an equivalent representation for the above defined process using the following conditional distributions:
%\begin{table}
%\begin{tabular}{p{4cm} p{3cm}}
%$\bm{\beta} | \gamma \sim \textnormal{GEM}(\gamma)$ & $\bm{\beta}' | \gamma' \sim \textnormal{GEM}(\gamma')$
%\end{tabular}
%\end{table}
%\begin{alignat}{2}
%\label{eq:mixtureMulti}
%&\bm{\beta} | \gamma \sim \textnormal{GEM}(\gamma) ~~~~~~&& \bm{\beta}' | \gamma' \sim \textnormal{GEM}(\gamma') \notag\\
%&\bm{\pi}_j | \alpha_j, \bm{\beta} \sim \textnormal{DP}(\alpha_j,\bm{\beta})~~~~~~ && z_{ji}|\bm{\pi}_j \sim \bm{\pi}_j \notag\\
%&\bm{\pi'}_{j'}| \alpha'_{j'}, \bm\beta' \sim \textnormal{DP}(\alpha'_{j'}, \bm\beta') ~~~~~~ &&z'_{j'i'}|\bm{\pi'}_{j'} \sim \bm{\pi'}_{j'} \notag\\
%&\phi_k|H \sim H ~~~~~ x_{j'i'}|z'_{j'i'} , (z_{ji})_{j=1,i =1}^{\infty,\infty}, (\phi_{k})^{\infty}_{k=1} &&\sim F(\phi_{z_{z'_{j'i'}i}})
%\end{alignat}
\begin{eqnarray}
\label{eq:mixtureMulti}
\beta \sim GEM(\gamma);\ \pi_{k'} \sim DP(\alpha, \beta) ;\ \phi_k \sim H,\ k,k'=1\ldots\infty \nonumber  \\
\beta' \sim GEM(\gamma')\ ; \pi'_{j} \sim DP(\alpha, \beta'),\ j=1\ldots M \nonumber \\
z'_{ji} \sim \pi'_j\ ;\ z_{ji} \sim \pi_{z'_{ji}} ;\ x_{ji} \sim F(\phi_{z_{ji}}),\ i=1\ldots n_j
\end{eqnarray}

This may be understood as first creating a entity-specific distributions $\pi_{k'}$ over topics using global topic popularities $\beta$, followed by creation of document-specific distributions $\pi'_j$ over entities using global entity popularities $\beta'$.
Using these parameters, the content of the $j^{th}$ document is generated by sampling repeatedly in $iid$ fashion an entity index $z'_{ji}$ using $\pi'_j$, a topic index $z_{ji}$ using $\pi_{z'_{ji}}$ and finally a word using $F(\phi_{z_{ji}})$.

Observe the connection with the ATM in Eqn. \ref{eqn:atm}.
The main difference is the the set of entities and topics is infinite. 
Separately, each document now has a distinct non-uniform distribution $\pi'_j$ over entities. 

Also, observe that we have preserved the HDP notation to the extent possible, to facilitate understanding.
To distinguish between variables corresponding to the two HDPs in the model, we use dashes ($'$) as superscripts on symbols corresponding to the outer HDP.
Going forward, we follow the same convention for naming variables in the nested CRF.

%\subsection{Nested Chinese Restaurant Franchise}
%\label{nCRF}
\vspace{0.05in}
\noindent
{\bf Nested Chinese Restaurant Franchise: }
In this section, we derive the predictive distribution for the next draw $\theta'_{ji}$ from the nHDP given previous draws, after integrating out $\{G'_j\}$ and $G'_0$, and then the predictive distribution for the draw $\theta_{ji}$ after integrating out $\{\theta'_{ji}\}$ and $G_0$.
We also provide an interpretation for then using two nested CRFs, corresponding to the inner and outer HDPs.
These will be useful for the inference algorithm that we describe in Section \ref{sec:inference}.

Let $\{\theta'_{ji}\}_{i=1}^{N_{j}}$ denote the sequence of draws from $G'_j$, and $\{\psi'_{jt'}\}_{t'=1}^{m'_{j\cdot}}$ denote the sequence of draws from $G'_0$.
Then the conditional distribution of $\theta'_{ji}$ given all previous draws after integrating out $G'_j$ looks as follows:
%\subsubsection*{Computing Marginals:}
%First consider the conditional distribution for $\theta'_{j'i'}$ given $\theta'_{j'1},$ $ \hdots,$ $\theta'_{j',i'-1}$ and $G'_0$, where $G'_{j'}$ is integrated out.
%\begin{equation}
%\label{thetaMulti}
%\begin{split}
%\theta'_{j'i'}|\theta'_{j'1}, & \hdots, \theta'_{j',i'-1}, \alpha'_{j'}, G'_0 \sim\\
%&\sum_{t'=1}^{m'_{j'\cdot}} \frac{n'_{j't'\cdot}}{i' - 1+\alpha'_{j'}} \delta_{\psi'_{j't'}} + \frac{\alpha'_{j'}}{i' - 1 +\alpha'_{j'}} G'_0
%\end{split}
%\end{equation}
\begin{equation}
\label{thetaMulti}
\begin{split}
\theta'_{ji}|\theta'_{j1:i-1}, \alpha'_{j}, G'_0 \sim
&\sum_{t'=1}^{m'_{j\cdot}} \frac{n'_{jt'\cdot}}{i - 1+\alpha'_{j}} \delta_{\psi'_{jt'}} + \frac{\alpha'_{j}}{i - 1 +\alpha'_{j}} G'_0
\end{split}
\end{equation}
where $n'_{jt'k'} = \sum_i \delta(\theta'_{ji}, \psi'_{jt'}) \delta(\psi'_{jt'}, G_{k'})$, $m'_{jk'}=\sum_{t'}\delta(\psi'_{jt'}, G_{k'})$. 
%A draw from the above mixture can be obtained by drawing from terms on RHS with probabilities given by the corresponding mixing proportions. 
Next, we integrate out $G'_0$, which is also distributed according to Dirichlet process:
\begin{equation}
\label{psiMulti}
\begin{split}
\psi'_{jt'}|\psi'_{11}, & \psi'_{12}, \hdots, \psi'_{21},  \hdots, \psi'_{j,t'-1}, \gamma', \text{HDP}(\bm\alpha, \gamma, H)\sim\\ &\sum_{k'=1}^{K'} \frac{m'_{\cdot j}}{m'_{\cdot\cdot} + \gamma'} \delta_{G_{k'}} + \frac{\gamma'}{m'_{\cdot\cdot} + \gamma'} \text{HDP}(\bm\alpha,\gamma,H)
\end{split}
\end{equation}

%To use the above equations to obtain samples of $\theta'_{ji}$, first sample $\theta'_{ji}$ for each $j$ and $i$ using (Eqn \ref{thetaMulti}). If new sample from $G'_0$ is needed, we use (Eqn \ref{psiMulti}) to obtain a new sample $G_{k'}$. Therefore, each $\theta'_{ji}$ variable gets a $G_{k'}$ assigned to it.
Observe that each $\theta'_{ji}$ variable gets assigned to one of the $G_{k'}$ variables.
Let $\{\theta_{ji}\}$ denote the sequence of draws from respective $\{\theta'_{ji}\}$ (i.e. from the corresponding $G_{k'}$), $\{\psi_{k't}\}$ the sequence of draws from $G_0$, and $\{\phi_k\}_{k=1}^\infty$ the sequence of draws from $H$. 
Let $\theta_{k':ji}$ denote the set of $\theta$ variables already drawn from $G_{k'}$ before sampling $\theta_{ji}$: 
$\theta_{k':ji} \equiv \{\theta_{j'i'}: \theta'_{j'i'} = G_k',\ \forall i',\ j' \leq j, \text{ and } i' < i,\ j' = j\}$. 
Then the conditional distribution of $\theta_{ji}$ given $\theta_{k':ji}$ and $G_0$, after integrating out $G_{k'}$ (corresponding to $\theta'_{ji}$) is as follows:
\begin{equation}
\label{thetanHDP}
\begin{split}
\theta_{ji}|\theta_{k':ji},  \alpha_0, G_0 \sim
\sum_{t=1}^{m_{k'\cdot}} \frac{n_{k't\cdot}}{i-1+\alpha_0} \delta_{\psi_{k't}} + \frac{\alpha_0}{n_{k'\cdot\cdot}+\alpha_0} G_0
\end{split}
\end{equation}
where $n_{k'tk}=\sum_{i}\delta(\theta_{k'i,\psi_{k't}})\delta(\psi_{k't},\phi_k)$, $m_{k'k}=\sum_{t}\delta(\psi_{k't},\phi_k)$ and dots indicate marginal counts. 
As $G_0$ is also distributed according to a Dirichlet Process, we can integrate it out similarly and write the conditional distribution of $\psi_{k't}$ as follows:
\begin{equation}
\label{psinHDP}
\begin{split}
\psi_{k't}|\psi_{11},  \psi_{12}, \hdots, \psi_{21},  \hdots, &\psi_{k't-1}, \gamma, H \sim \sum_{k=1}^{K} \frac{m_{\cdot k}}{m_{\cdot\cdot} + \gamma} \delta_{\phi_{k}} + \frac{\gamma}{m_{\cdot\cdot} + \gamma} H
\end{split}
\end{equation}
Note that both conditional distributions for $\theta'_{ji}$ and $\theta_{ji}$ are similar to that for CRF (Eqns. \ref{eqn:thetaHDP} and \ref{eqn:psiHDP}).
We interpret these two distributions as a \textit{nested Chinese Restaurant Franchise}, involving one inner CRF and one outer CRF.

Consider a set of outer restaurants, one corresponding to each group.
Customers entering each of these restaurants select a table $\theta'_{ji}$ according a group specific CRP (Eqn \ref{thetaMulti}).
The restaurants share a common set of inner restaurants $\{G_{k'}\}$.
Inner restaurant are assigned to the tables of each outer restaurant according to another CRP (Eqn \ref{psiMulti}).
Next, the customers go to the inner restaurant assigned to them (at the outer restaurant) and select a table $\theta_{ji}$ according to the inner restaurant specific CRP (Eqn \ref{thetanHDP}).
These inner restaurants share a common menu of dishes $\{\phi_k\}$.
Dishes are assigned to the tables of each inner restaurant according to another CRP (Eqn \ref{psinHDP}).

Let $t'_{ji}$ be the (outer table) index of the $\psi'_{jt'}$ associated with $\theta'_{ji}$, and let $k'_{jt}$ be the (inner restaurant) index of the $G_{k'}$ associated with $\psi'_{jt'}$.
Let $t_{ji}$ be the (inner table) index of the $\psi_{k't}$ associated with $\theta_{ji}$, and let $k_{k't}$ be the (dish) index of the $\phi_k$ associated with $\psi_{k't}$.
Then the two conditional distributions above can also be written in terms of the indexes $\{t'_{ji}\}, \{k'_{jt'}\}$, $\{t_{ji}\}$ and $\{k_{k't}\}$ instead of referring to the distributions directly.
%A draw from the above mixture can be obtained by drawing from terms on RHS with probabilities given by the corresponding mixing proportions. 
For each outer restaurant $j$ and its customer $i$, we draw $\theta'_{ji}$ using (Eqn. \ref{thetaMulti}). If the first summation is chosen, we set $\theta'_{ji} = \psi'_{jt'}$ and let $t'_{ji} = t'$ for the chosen $t'$. If the second term is chosen, then we increment $m'_{j\cdot}$ by one, draw $\psi'_{jm'_{j\cdot}} \sim G'_0$ using (Eqn \ref{psiMulti}) and set  $\theta'_{ji} = \psi'_{jm'_{j\cdot}}$ and $t'_{ji} = m'_{j\cdot}$. 
If we draw $\psi'_{jt'}$ via choosing a summation term, we set $\psi'_{jt'}= G_{k'}$ and let $k'_{jt'} =k'$ for the chosen $k'$.
If the second term is chosen, then we increment the current distinct entity count $M$ by one, draw $G_M \sim \text{HDP}(\bm\alpha,\gamma,H)$ and set  $\psi'_{jt'} = G_M$ and $k'_{jt'} = M$. 
Next, we similarly draw samples of $\theta_{ji}$ for each $j$ and $i'$ using (Eqn. \ref{thetanHDP}). If new sample from $G_0$ is needed, we use (Eqn. \ref{psinHDP}) to obtain a new sample $\psi_{k't}$. 
%Next for each $j$ and $i$ we draw $\theta_{ji}$ using (Eqn. \ref{thetaHDP}). If the first summation is chosen , we set $\theta_{ji} = \psi_{jt}$ and let $t_{ji} = t$ for the chosen $t$. If the second term is chosen, then we increment $m_{j\cdot}$ by one, draw $\psi_{jm_{j\cdot}} \sim G_0$ using (Eqn \ref{psiHDP}) and set  $\theta_{ji} = \psi_{jm_{j\cdot}}$ and $t_{ji} = m_{j\cdot}$. 
%If we draw $\psi_{jt}$ via choosing a summation term, we set $\psi_{jt}= \phi_k$ and let $k_{jt} =k$ for the chosen $k$. If the second term is chosen, we increment $K$ by 1 and draw $\phi_K \sim H$ and set $\psi_{jt} = \phi_K$ and $k_{jt} = K$.

%To use the above equations to obtain samples of $\theta'_{ji'}$, first sample $\theta'_{ji'}$ for each $j$ and $i'$ using (\ref{thetaMulti}). If new sample from $G'_0$ is needed, we use (\ref{psiMulti}) to obtain a new sample $\psi'_{jt'}$. 
%
%Then for each inner restaurant $j$ and its $i$th customer (which is a table from outer restaurant), we use (\ref{thetaHDP}) to sample $\theta_{ji}$ and if a new sample from $G_0$ is required, then (\ref{psiHDP}) is used to obtain a new sample $\psi_{jt}$ and set $\theta_{ji} = \psi_{jt}$.


%In this metaphor, we consider two sets of restaurants, one set of inner restaurants and another distinct set of outer restaurants. 

%The set of inner restaurants share a global menu of dishes and the set of outer restaurants fetch the dishes from the inner restaurants shared across the outer restaurants. At each table in each outer restaurant, the first customer gets a dish from an inner restaurant of his choice which is shared by everyone sitting at that table. Note that, in this setup, the tables (or their first customer) of outer restaurants are the customers in the inner restaurants. 
 
%Each outer restaurant corresponds to a groups and its customers represent the factors $\theta'_{j'i'}$. The inner restaurants correspond to the set of entities shared by the groups. For brevity, we reuse the description and notations of restaurants in Chinese restaurant franchise (in \S~\ref{sec:crf}) for the set of inner restaurants. Therefore,  let $G_j \sim$ HDP$(\alpha_j, \gamma, H)$ denote the distribution for entity $j$. Let  $\psi'_{j't'}$ denote inner restaurant chosen by the table $t'$ in outer restaurant $j'$. We use the notations $\theta_{ji}$ and $\psi_{jt}$ from the CRF metaphor. In this setting, the notation $\theta_{ji}$ correspond to the $i$-th customer, which is a table from outer restaurant, in inner restaurant $j$.


%Note that each $\theta'_{j'i'}$ is associated with one $\psi'_{j't'}$, which in turn is associated with one $G_j$.
% and its $\psi_{jt}$. While a $\psi_{jt}$	is associated with one $\phi_k$
 %Let $t'_{j'i'}$ be the index of $\psi'_{j't'}$ associated with $\theta'_{j'i'}$ and $j_{j't'}$ be the index of $G_j$ (inner restaurant) associated with $\psi'_{j't'}$. 
%Let $t_{k'i}$ be the index of $\theta_{k'i}$ (counter) associated with the $i$-th table assigned to the chef with index $k'$. Let $k_{k't}$ be the index of $\phi_k$ associated with $\psi_{k't}$. 
% Therefore, customer $i'$ of outer restaurant $j'$ sits at table $t'_{j'i'}$ and the order of table $t'$ gets a dish from inner restaurant $j$ and specifically the table $t$ in that inner restaurant which serves dish $k_{jt}$. 

%We maintain the counts of dishes and customers and tables of the two franchise. We use the notation $n'_{j't'j}$ to denote the number of customers of outer restaurant $j'$ at table $t'$ placing their order from inner restaurant $j$ and $m'_{j'j}$ denotes the number of tables of outer restaurant $j'$ that have place their order from inner restaurant $j$. Other counts are the same as those used in Chinese restaurant franchise. Note that marginal counts are represented by dots.

%Let $n_{k'tk}$ denote the number of tables assigned to counter $t$ of chef $k'$ serving dish $k$ and $m_{k'k}$ denote the number of counters of chef $k'$ serving dish $k$. 

%\subsection{Infinite limit of finite mixture models}
%Consider the following collections of finite mixture models, where $\beta$ is a global vector of mixing proportions and $\pi_a$ is a group-specific
%
%$$\bm{\beta}|\gamma \sim \textnormal{Dir}(\gamma/L, \hdots, \gamma/L); ~~~ \phi_k | H \sim H; ~~~ k_{k't} | \beta \sim \beta$$
%$$\pi_{k'}| \alpha \sim  \textnormal{Dir}(\alpha/T, \hdots, \alpha/T); ~~~ t_{k'_{{jt'}t'}} |\pi_{k'} \sim \pi_{k'}  $$
%$$\bm{\beta'}|\gamma' \sim \textnormal{Dir}(\gamma'/L', \hdots, \gamma/L'); ~~~ k'_{jt'} | \beta' \sim \beta' $$
%$$\pi'_j| \alpha'_j \sim  \textnormal{Dir}(\alpha'^*/T', \hdots, \alpha'^*/T'); ~~~ t'_{ji'} |\pi_{j} \sim \pi_{j}$$
%$$ x_{ji'} | t'_{ji'}, (\langle k', t\rangle_{jt'})^{T'}_{t'=1}, (k_{k't})_{k',t=1}^{L',T} , (\phi_k)_{k=1}^L \sim$$ $$F(\phi_{k_{k't_{jt'_{ji'}}}})$$
%
%As $T' \rightarrow \infty, L' \rightarrow \infty, T \rightarrow \infty$ and $L \rightarrow \infty$, the limit of this model is the entity-topic model defined above for multiple entities per document.


==> SingleAuthorModel.tex <==
%We propose nonparametric Bayesian approach for modeling entities associated with the documents, where each entity is associated with a mixture model. We define an appropriate non-parametric prior and present a stick-breaking construction, a Chinese restaurant process representation, and a representation in terms of a limit of finite mixture models. To start with, let us assume that an entire document is associated with a single entity.

We now present our nested HDP model for non-parametric entity topic analysis.
We first present the model where each group or document is associated with a single entity, then extend it for multiple entities.

%\subsection{Single-Entity Documents}
%\label{single}
\vspace{0.05in}
\noindent
{\bf Single-Entity Documents: }
Recall that the nDP is unsuitable for entity-topic analysis, since the entity distributions does not share topic atoms.
This can be modified by first creating a set of entity distributions $\{G_{k'}\}_{k'=1}^\infty$ such that they share atoms.
One way to do this %while retaining flexibility 
is to follow the HDP construction: 
\begin{equation}
\label{gS}
G_{k'}\sim HDP(\{\alpha_{k'}\},\gamma,H)
\end{equation}
This can be followed by drawing each group specific distribution from a mixture over the $G_{k'}$s:
\begin{equation}
\label{gJd}
G'_j\sim G'_0 \equiv \sum_{k'=1}^\infty \beta'_{k'}\delta_{G_{k'}},\ \beta'\sim GEM(\gamma')
\end{equation}
Using Eqn. \ref{eq:dpStick}, we observe that $G'_0 \sim DP(\gamma',HDP($ $\{\alpha_{k'}\},\gamma,H))$.
Observe the relationship with the nDP (Eqn. \ref{eqn:ndp:dpfamily}).
Like the nDP, this also defines a distribution over the space of distributions on distributions.
But, instead of a DP base distribution for the outer DP, we have achieved sharing of atoms using a HDP base distribution.
We will write $G'_j\sim \mbox{DP-HDP}(\gamma',\{\alpha_{k'}\},\gamma,H)$.

Sampling $G'_j$ may be imagined as choosing the entity for document $j$. 
As before, $G'_j$ can now be used as prior for sampling topics $\{\theta_{ji}\}$ for individual words in document $j$, followed by sampling of the words themselves, using Eqn \ref{eq:mixture}.
%\begin{equation}
%\label{eq:DP-HDPmm}
%\theta_{ji}\sim G_j,\ x_{ji}\sim F(\theta_{ji})
%\end{equation}
We will call this the DP-HDP mixture model. 
 
%The process is a distribution over space of distributions over a set of random probability measures over $(\Theta, \mathcal{B})$. The process first defines a set of random probability measures $G_j$, one for each entity, from a hierarchical Dirichlet process, HDP$(\bm\alpha, \gamma, H)$. 

 %$$G_j|\alpha_j, \gamma, H \sim \textnormal{HDP}(\alpha_j, \gamma, H) ~~~~~ \textnormal{for each entity }j.$$
%Next, the process defines a space of distributions, $G^*_0$, on the above set of random probability measures over $(\Theta, \mathcal{B})$ as follows:
%\begin{equation}
%\label{gS}
%G^*_0|\gamma^*,\bm\alpha,\gamma, H \sim \text{DP}(\gamma^*, \text{HDP}(\bm\alpha, \gamma, H))
%\end{equation}
%The collection of distributions $\{G^*_1, \hdots, G^*_{j'}\}$ is then sampled independently from the above defined space of distributions
%\begin{equation}
%\label{gJd}
%G^*_{j'} \stackrel{iid}{\sim} G^*_0 \textnormal{~~for each group } j'.
%\end{equation}
%The hyperparameters of the above process consist of the baseline probability measure $H$, and the concentration parameters $\gamma, \bm\alpha$ and $\gamma^*$. 
%The process can be used as the prior distribution over the factors of the grouped data. For each group $j'$, let $\theta^*_{j'1}, \theta^*_{j'2}, \hdots$ be i.i.d. random variables distributed as $G^*_{j'}$. Each $\theta^*_{j'i'}$ is a factor corresponding to a single observation $x_{j'i'}$. 
%The likelihood is given by
%\begin{alignat}{2}
%\label{eq:mixtureSingle}
%&\theta^*_{j'i'} |G^*_{j'} \sim G^*_{j'} ~~ &&\textnormal{for each } {j'} \textnormal{ and } i', \notag\\
%&x_{{j'}i'} |\theta^*_{{j'}i'} \sim F(\theta^*_{{j'}i'}) ~~~&&\textnormal{for each } {j'} \textnormal{ and } i'.
%\end{alignat}

%\subsubsection{The stick-breaking construction}
%Using the stick-breaking construction, we can express the global measure $G_0$ distributed as Dirichlet process:
%%Given the base measure $G_0$ is distributed as a Dirichlet process, it can be expressed as follows
%$$G_0 = \sum_{k=1}^\infty \beta_k \delta_{\phi_k}, $$
%where $\phi_k \sim H$ independently and $ \beta = (\beta_k)_{k=1}^\infty \sim $ GEM$(\gamma)$ are mutually independent. Similar to HDP, each $G^*_a$ can be written as follows:
%\begin{equation}
%\label{gAstick}
%G^*_a = \sum_{k=1}^\infty \pi_{ak} \delta_{\phi_k},
%\end{equation}
%where $\pi_a= (\pi_{ak})_{k=1}^\infty \sim \textnormal{DP}(\alpha, \beta)$ are mutually independent. Again, 

%Given that $G^*_0$ is distributed as Dirichlet process, it can be expressed using the following stick-breaking representation:
%\begin{equation}
%\label{gSstick}
%G^*_0= \sum_{j=1}^\infty \beta_{j}^* \delta_{G_j},
%\end{equation}
%where $ \bm\beta^* = (\beta^*_j)_{j=1}^\infty \sim $ GEM$(\gamma^*)$ and $G_j \sim \text{HDP}(\alpha_j, \gamma, H)$ (see (\ref{gJstick}) for stick-breaking expression of $G_j$).
%\begin{equation}
%\label{gJdstick}
%G^*_{j'} \stackrel{iid}{\sim} G^*_0 \textnormal{~~for each } j',
%\end{equation}
%and therefore, each $G^*_{j'}$ corresponds to one of the entity distributions $G_j$. 



%\subsection{Single Entity Model with Document specific Topic Mixture}
%In the above model, the document identity is not maintained and only the entity-specific distribution is used while sampling the topics for the words in a document. Usually documents associated with the same entity have quite different distribution of topics. The single entity model described in previous section (\S~\ref{single}) will fail to capture this aspect as it assumes that all the documents associated with an entity share a common distribution over topics. In order to use the document-specific characteristics, we define another set of random probability measures $G'_{j'}$, one for each group $j'$, with the probability measure corresponding to the associated entity $G^*_{j'}$ as the base measure. As defined in (\ref{gJd}), $G^*_{j'} \sim G^*_0$ picks the entity specific distribution $G_j$, and hence, we define $G'_{j'}$ as follows
%$$G'_{j'}|\alpha', G^*_{j'} \sim  \textnormal{DP}(\alpha', G^*_{j'}) ~~~~~~~~ \text{for each } j' $$
%Like the earlier single entity model, the above process can be as prior distribution for the factors of grouped data (refer (\ref{eq:DP-HDPmm})).


%For each ${j'}$, let $\theta'_{j'1}, \theta'_{j'2}, \hdots$ be i.i.d. random variables distributed as $G'_{j'}$. In this model, $\theta'_{j'i}$ is a factor corresponding to  observation $x_{j'i}$. Therefore, likelihood is given by
%$$\theta'_{j'i} |G'_{j'} \sim G'_{j'} \textnormal{~~for each } j' \textnormal{ and } i,$$
%$$x_{j'i} |\theta'_{j'i} \sim F(\theta'_{j'i}) \textnormal{~~for each } j' \textnormal{ and } i.$$


==> inference.tex <==
\section{Inference}
\label{sec:inference}

We use Gibbs sampling for inference. Similar to the approach followed in HDP \cite{HDP}, instead of sampling the latent variables $\theta'_{ji'}, \psi'_{jt'}, \theta_{k'i}$ and $\psi_{ k't}$, their indices are sampled. Therefore, the variables that need to be sampled as a part of the Gibbs sampling iteration are  all the instances of $t'_{ji'}$ (tables), $k'_{jt'}$ (chefs), $t_{ki'}$ (counters) and $k_{k't}$ (dishes).

We use a joint sampling scheme for chefs  $k'_{jt'}$ and their counters $t_{ki'}$, where we jointly sample a chef and its counter for a given organization $j$ and its table $t'$. Therefore, for simplicity, we use the notation $\langle k', t\rangle_{jt'} \sim (k'_{jt'}, t_{jt'})$ to denote the chef and its counter associated with $t'$ table of organization $j$.
%
%We additionally introduce $t_{jt'}$ to denote the counter index corresponding to the specific chef $k'_{jt'}$ for table $t'$ in organization $j$.(We had used the notation of $t_{k'i}$ earlier, 
%to refer to the chef's specific counter index of $i^{th}$ table assigned to chef $k'$. However, while sampling, we sample the counter index for each table in each organization. Hence the new notation is introduced for simplicity.).
% We note that the variables $k'_{jt'}$ and $t_{jt'}$ cannot be sampled independently.
%This is because the counter index $t_{jt'}$ is valid only in the context of a specific chef  $k'_{jt'}$. Hence we do a joint sampling of variables $k'_{jt'}$ and $t_{jt'}$ where ever appropriate. 

Let $\textbf{x} = (x_{ji'} :$ all $j,i'),$ 
$\textbf{x}_{jt'} = (x_{ji'}:$ all $i'$ with $t'_{ji'} = t'),$ 
%\textbf{x}_{k'} = (x_{jt'}:$ all $j,t'$ with $k'_{jt'} = k'),
$\textbf{x}_{k't} = (\textbf{x}_{jt'}:$ all $j,t'$ with $\langle k',t\rangle_{jt'} = \langle k',t\rangle),$  
%$t_{k'_{jt'}t'} = t),$ 
$\textbf{t}' = (t'_{ji'} :$ all $j,i'),$ 
$\langle\textbf{k}', \textbf{t}\rangle = (\langle k',t\rangle_{jt'} :$ all $j,t'),$ 
%$\textbf{k}' = (k'_{jt'} :$ all $j,t'),$ 
%$\textbf{t} = (t_{jt'} :$ all $j, t'),$ 
$\textbf{k} = (k_{k't} :$ all $\langle k',t\rangle),$ 
$\textbf{z} = (z_{ji'} :$ all $j,i'),$ 
$\textbf{m}' = (m'_{jk'} :$ all $j,k'),$ 
$\textbf{m} = (m_{k'k} :$ all $k,k).$  

Further, when a set is subscripted with hyphenated indices, the set of variables corresponding to the unhyphenated indices is to be removed from the superset with all possible values for the indices.
For example, $\textbf{x}_{-k't}$ indicates $\{\textbf{x} - \textbf{x}_{k't}\}$. Similarly, $t'_{-ji'}$ indicates, $\{\textbf{t}' - t'_{ji'}\}$ .


Let $F(\theta)$ have density $f(\cdot|\theta)$ and $H$ have density $h(\cdot)$.
We denote the conditional density of $x_{ji'}$ under mixture component $k$ given all data items except $x_{ji'}$ using the notation  $f^{\textbf{x}_{-ji'}}_{k}(x_{ji'})$ in HDP \cite{HDP}. 
Similarly,  $f^{\textbf{x}_{-ji'}}_{k^{new}}(x_{ji'})$ denotes the conditional density of  $x_{ji'}$, given a new mixture component $\phi_k^{new}$ is chosen, with only one customer associated with it.  
$f^{\textbf{x}_{-jt'}}_{k}(\textbf{x}_{jt'})$ and $f^{\textbf{x}_{-k't}}_{k}(\textbf{x}_{k't})$  denote the conditional density of $\textbf{x}_{jt'}$ and  $\textbf{x}_{k't}$ under mixture component $k$ respectively. 
$f^{\textbf{x}_{-jt'}}_{k^{new}}(\textbf{x}_{jt'})$ and $f^{\textbf{x}_{-k't}}_{k^{new}}(\textbf{x}_{k't})$  are the conditional density of $\textbf{x}_{jt'}$ and $\textbf{x}_{k't}$  with a new mixture componant respectively.

Let ${\phi} = (\phi_1, \cdots , \phi_k)$. The evaluation of various conditional densities above can be carried out by integrating out ${\phi}$, as shown in HDP \cite{HDP}.\\


{\bf \emph{  Sampling Table assignments $t'_{ji'}$}}
\begin{equation}
\label{inference_td}
\begin{split}
&p(t'_{ji'} = t' | \textbf{t}'_{-ji'}, {\bf k'}, {\bf t} , {\bf k}, {\bf x}) \propto  \\
&\begin{cases}
n'_{jt'.} \hspace{2mm} f_{k_{k'_{jt'}t_{jt'}}}^{\textbf{x}_{-ji'}}(x_{ji'}) \hfill \text{existing $t'$}\\
\alpha'_j \hspace{2mm} p(x_{ji'} | t'_{ji'}=t'^{new}, t'_{-ji'}, \bf{k'}, \bf{t}, \bf{k}, \textbf{x}_{-ji'}) \hfill \text{new $t'$}
\end{cases}
\end{split}
\end{equation}
Let $f_{t^{new}}^{\textbf{x}_{-ji'}}(x_{ji'})$, the probability of observing $x_{ji'}$, given that the entire vector is associated with a newly created counter, be defined as follows by marginalizing 
over all possible assignments of a dish to the new counter.
\begin{equation}
\label{inference_ftnew_jid}
\begin{split}
 f_{t^{new}}^{\textbf{x}_{-ji'}}(x_{ji'}) = \sum_{k=1}^{K} \frac{m_{\cdot k}}{m_{\cdot \cdot} + \gamma}  f_{k}^{\textbf{x}_{-ji'}}(x_{ji'}) +\frac{m_{ \cdot \cdot }}{m_{\cdot \cdot} + \gamma}  f_{k^{new}}^{\textbf{x}_{-ji'}}(x_{ji'})
\end{split}
\end{equation}
When a new table $t'$ is created in organization j, it can get an existing  chef $k'$ and an existing counter $t$, or an existing chef $k'$  with a new counter, or a new chef.
Hence, to compute $p(x_{ji'} | t'_{ji'}=t'^{new}, \textbf{t}'_{-ji'}, {\bf k'}, {\bf t}, {\bf k}, \textbf{x}_{-ji'}) $, we sum over all possible assignments of chef $k'$ and counter $t$

\begin{equation}
\label{inference_td_new}
\begin{split}
 p(x_{ji'} | t'_{ji'}=t'^{new}, \textbf{t}'_{-ji'}, {\bf k'}, {\bf t}, {\bf k}, \textbf{x}_{-ji'}) = \\
\sum_{k'=1}^{A} \sum_{t=1}^{m_{k'\cdot}} \frac{m'_{\cdot k'}}{m'_{\cdot\cdot}+\gamma^*}  \frac{n_{k't\cdot}}{n_{k' \cdot \cdot} + \alpha} f_{k_{k't}}^{\textbf{x}_{-ji'}}(x_{ji'}) +\\
\sum_{k'=1}^{A} \frac{m'_{\cdot k'}}{m'_{\cdot\cdot}+\gamma^*} \frac{\alpha}{n_{k' \cdot \cdot} + \alpha}  f_{t^{new}}^{\textbf{x}_{-ji'}}(x_{ji'}) + \\
\frac{\gamma^*}{m'_{\cdot \cdot} + \gamma^*} f_{t^{new}}^{\textbf{x}_{-ji'}}(x_{ji'})
\end{split}
\end{equation}

Further, when a new table $t'^{new}$ is created, a chef $k'_{jt'^{new}}$ and a counter $t_{jt'^{new}}$ are jointly sampled for it as follows
 
\begin{equation}
\label{inference_td_new_kdt}
\begin{split}
 p(k'_{jt'^{new}} = k', t'_{jt'^{new}} =t | \textbf{k}'_{-jt'^{new}}, \textbf{t}'_{-jt'^{new}}, {\bf k}, \textbf{x}_{-ji'}) \propto  \\
\begin{cases}
\frac{m'_{\cdot k'}}{m'_{\cdot\cdot}+\gamma^*}  \frac{n_{k't\cdot}}{n_{k' \cdot \cdot} + \alpha} f_{k_{k't}}^{\textbf{x}_{-ji'}}(x_{ji'}) \hfill \text{Existing $k',t$}\\
\frac{m'_{\cdot k'}}{m'_{\cdot\cdot}+\gamma^*} \frac{\alpha}{n_{k' \cdot \cdot} + \alpha}  f_{t^{new}}^{\textbf{x}_{-ji'}}(x_{ji'})  \hfill \text{Existing $k'$, new $t$}\\
\frac{\gamma^*}{m'_{\cdot \cdot}  + \gamma^*} f_{t^{new}}^{\textbf{x}_{-ji'}}(x_{ji'}) \hfill \text{new $k'$,new $t$}
\end{cases}
\end{split}
\end{equation}

In this process, when a new chef is selected for $k'_{jt'^{new}}$, a new counter is automatically created for this chef. A dish $k_{k't^{new}}$ is assigned to this counter as follows.

\begin{equation}
\label{inference_k_dt}
\begin{split}
 p(k_{k't^{new}} = k |\textbf{k}_{-k't^{new}} , {\bf \textbf{x}_{-ji'}}) \propto  \\
\begin{cases}
m_{\cdot k}  f_{k}^{\textbf{x}_{-ji'}}(x_{ji'}) \hfill \text{Existing $k$}\\
\gamma f_{k^{new}}^{\textbf{x}_{-ji'}}(x_{ji'})  \hfill \text{new $k$}
\end{cases}
\end{split}
\end{equation}

{\bf \emph{ Sampling Chef and Counter assignments $k'_{jt'}$, $t_{jt'}$}}
We provide an update rule similar to equation \ref{inference_td_new_kdt} for the joint sampling of variables $k'_{jt'}$ and $t_{jt'}$.

Let $f_{t^{new}}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'})$, the likelihood of observing $x_{jt'}$, given that it gets is dish from a newly created counter, be defined as follows.

\begin{equation}
\label{inference_ftnew_jtd}
\begin{split}
 f_{t^{new}}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'}) = \sum_{k=1}^{K} \frac{m_{\cdot k}}{m_{\cdot \cdot} + \gamma}  f_{k}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'}) +\frac{m_{ \cdot \cdot }}{m_{\cdot \cdot} + \gamma}  f_{k^{new}}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'})
\end{split}
\end{equation}

Now we can sample $k'_{jt'}$ and $t_{jt'}$ as follows.
\begin{equation}
\label{inference_kdt_joint}
\begin{split}
 p(k'_{jt'} = k', t_{jt'} =t | \textbf{k}'_{-jt'}, \textbf{t}'_{-jt'}, {\bf k}, {\bf x_{-jt'}}) \propto  \\
\begin{cases}
\frac{m'_{\cdot k'}}{m'_{\cdot\cdot}+\gamma^*}  \frac{n_{k't\cdot}}{n_{k' \cdot \cdot} + \alpha} f_{k_{k't}}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'}) \hfill \text{Existing $k',t$}\\
\frac{m'_{\cdot k'}}{m'_{\cdot\cdot}+\gamma^*} \frac{\alpha}{n_{k' \cdot \cdot} + \alpha}  f_{t^{new}}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'})  \hfill \text{Existing $k'$, new $t$}\\
\frac{\gamma^*}{m'_{\cdot \cdot} + \gamma^*} f_{t^{new}}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'}) \hfill \text{new $k'$}
\end{cases}
\end{split}
\end{equation}

Again, if a new counter has been sampled, a dish $k_{k't^{new}}$ is selected for it as follows

\begin{equation}
\label{inference_kdt_k}
\begin{split}
 p(k_{k't^{new}} = k |\textbf{k}_{-k't^{new}} , {\bf x_{-jt'}}) \propto  \\
\begin{cases}
m_{\cdot k}  f_{k}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'}) \hfill \text{Existing $k$}\\
\gamma f_{k^{new}}^{\textbf{x}_{-jt'}}(\textbf{x}_{jt'})  \hfill \text{new $k$}
\end{cases}
\end{split}
\end{equation}


{\bf \emph{ Sampling dish assignments $k_{k't}$}}

Finally, to sample a dish for the counter, the conditional distribution of $k_{k't}$ follows 
\begin{equation}
\label{inference_k}
\begin{split}
 p(k_{k't} = k |\textbf{k}_{-k't} , {\bf x_{-k't}}) \propto  \\
\begin{cases}
m_{\cdot k}  f_{k}^{\textbf{x}_{-k't}}(\textbf{x}_{k't}) \hfill \text{Existing $k$}\\
\gamma f_{k^{new}}^{\textbf{x}_{-k't}}(\textbf{x}_{k't})  \hfill \text{new $k$}
\end{cases}
\end{split}
\end{equation}

The inference procedure during each Gibb's iteration is shown in Algorithm \ref{inference_alg}

\begin{algorithm}
%\caption{Inference : Gibbs Iteration}
{\fontsize{7}{7}\selectfont
\begin{algorithmic}
\label{inference_alg}
 \For{Organization $j$ from $1$ to $N$}
 \For{customers $i$ from $1$ to $n'_{j..}$}
         \State Pick a table $t'_{ji'}$ using equation \ref{inference_td}
         \If{New table in $j$ } 
 	      \State Assign chef $k'_{jt'^{new}}$ ,counter $t_{jt'^{new}}$ with equation \ref{inference_td_new_kdt}
 	      \If{New Counter}
 	          \State Assign a dish $k_{k't^{new}}$ from equation \ref{inference_k_dt}
 	      \EndIf       
 	\EndIf
 \EndFor
 \EndFor
 \For{Organization $j$ from $1$ to $N$}
 \For{Tables $t'$ from $1$ to $m'_{j.}$}
         \State Assign a chef $k'_{jt'}$ and a counter $t_{jt'}$ using equation \ref{inference_kdt_joint}
 	\If{New Counter}
 	     \State Assign a dish $k_{k't^{new}}$ from equation \ref{inference_kdt_k}
 	\EndIf       
 	
 \EndFor
 \EndFor
 \For{Chef $k'$ from $1$ to $A$}
 \For{Counters $t$ from $1$ to $m_{k'.}$}
 	     \State Assign a dish $k_{k't}$ from equation \ref{inference_k}
 \EndFor
 \EndFor
\end{algorithmic}}
\end{algorithm}



==> inference_direct.tex <==
\section{Inference for Nested HDP}
\label{sec:inference}

We use Gibbs sampling for approximate inference as exact inference is intractable for this problem. 
The conditional distributions for the nCRF scheme lend themselves to an inference algorithm, 
where we sample {$t'_{ji}$}, {$t_{ji}$}, {$k'_{jt'}$} and {$k_{k't}$}. The conditionals for these variables are similar to 
those in equation \ref{thetaMulti}, \ref{thetanHDP}, \ref{psinHDP} and \ref{psiMulti} respectively. 
However, in such an approach, there exists a tight coupling between the variables {$t'_{ji}$}, {$t_{ji}$} and {$k'_{jt'}$}, which would call for
computationally expensive joint sampling of variables.

Instead we adopt a technique similar to the direct sampling scheme in HDP\cite{HDP} where variables $G_0$ and $G'_0$ are explicitly sampled instead of being 
integrated out, by sampling the stick breaking weights $\beta$ and $\beta'$ respectively. Further, we directly sample {$z_{ji}$} (the topic) 
and {$z'_{ji}$} (the author) for each word in document j avoiding explicit table assignments to the {$t'_{ji}$} and {$t_{ji}$} variables. 
However, in order to sample $\beta$ and $\beta'$, the table information is maintained in the form of the number of tables in each outer 
and inner restaurant, {$m'_{jk'}$} and {$m_{k'k}$} respectively.
Thus the latent variables that need to be sampled in our Gibbs sampling scheme are {$z_{ji}$}, {$z'_{ji}$}, $\beta$, $\beta'$, 
{$m_{jk'}$} and {$m_{k'k}$}.

We introduce the following notation for the rest of this section. 
Let $\textbf{x} = (x_{ji} :$ all $j,i),$ 
${\bf x_{-ji}} = (x_{j'i'} : j' \neq j , i' \neq i),$
$\textbf{m} = (m_{k'k} :$ all $k',k),$  
$\textbf{m}' = (m'_{jk'} :$ all $j,k'),$ 
$\textbf{z} = (z_{ji} :$ all $j,i),$ 
$\textbf{z}' = (z'_{ji} :$ all $j,i),$ 
${\bf z_{-ji}} = (z_{j'i'} : j' \neq j , i' \neq i),$
${\bf z'_{-ji}} = (z'_{j'i'} : j' \neq j , i' \neq i),$ 
$\beta_{new}= \sum_{k=K+1}^{\infty} \beta_k$
and $\beta'_{new}= \sum_{k'=K'+1}^{\infty} \beta'_{k'}$


%\vspace*{0.1in} \noindent
{\bf Sampling {$z_{ji}$}: } The conditional distribution for topic index $z_{ji}$ is
\begin{equation*}
%\label{inference_zji}
\begin{split}
 p(z_{ji} = z | {\bf z_{-ji}} ,  {\bf z'_{-ji}}, z'_{ji} = z',  {\bf m}, {\bf m'}, \beta, \beta', {\bf x}) 
 \propto p(z_{ji} = z| {\bf z_{-ji}}, z'_{ji} = z' ) p(x_{ji} | z_{ji} = z, {\bf x_{-ji}}) 
 \end{split}
\end{equation*}

For existing topics, $p(z_{ji} = z| {\bf z_{-ji}}, z'_{ji} = z' )$ can be split into two terms. One from 
 picking any of the existing inner tables from entity $z'$ with topic $z$ and one from creating a new inner table in entity $z'$ and 
 assigning the topic $z$ to it. For a new topic, a new inner table is always created in entity $z'$. Hence, 
 \begin{equation}
\label{inference_zji_a}
 p(z_{ji} = z| {\bf z_{-ji}}, z'_{ji} = z' ) \propto 
 \begin{cases}
\frac{n_{k'.k} + \alpha \beta_k}{n_{k'.}+\alpha}   \hfill \text{  Existing $z$}\\
\frac{\alpha \beta_{new}}{n_{k'..}+\alpha}   \hfill \text{  New topic $z$}
 \end{cases}
\end{equation}

The other term $p(x_{ji} | z_{ji} = z, {\bf x_{-ji}}) $ is the conditional density of $x_{ji}$ under topic $z$ given all data items except $x_{ji}$. 
Assuming each topic is sampled from a V dimensional symmetric dirichlet prior over the vocabulary with parameter $\eta$, i.e $\phi_k \sim Dir(\eta)$, the above probability can be simplified to the following expression, by integrating out $\phi$.
 \begin{equation*}
%\label{inference_zji_b}
 p(x_{ji} = w | z_{ji} = z, {\bf x_{-ji}})  \propto \frac{ n_{zw} + \eta}{n_z. +  V \eta}
\end{equation*}
where $n_{zw}$ is the number of occurances of topic z with word w in the vocabulary.

%\vspace*{0.1in}\noindent
{\bf Sampling {$z'_{ji}$}: } The conditional distribution for the entity index $z'_{ji}$ is 
\begin{equation*}
%\label{inference_z'ji}
\begin{split}
 p(z'_{ji} = z' | {\bf z'_{-ji}} ,  {\bf z_{-ji}}, z_{ji} = z,  {\bf m}, {\bf m'}, \beta, \beta', {\bf x}) 
 \propto p(z'_{ji} = z| {\bf z'_{-ji}}) p(z_{ji} = z| {\bf z_{-ji}}, z'_{ji} = z' )
 \end{split}
\end{equation*}

 Again, $p(z_{ji} = z| {\bf z_{-ji}}, z'_{ji} = z' )$ can be split into two terms. One from 
 picking an existing outer table with entity $z'$ and one from creating a new outer inner table and assigning the entity $z'$ to it. 
 Further, creation of a new entity always involves the creation of a new outer table. Hence, 
 \begin{equation*}
%\label{inference_z'ji_a}
 p(z'_{ji} = z'| {\bf z'_{-ji}} ) \propto 
 \begin{cases}
\frac{n'_{j.k'} + \alpha' \beta'_{k'}}{n'_{j..}+\alpha'} \hfill \text{Existing $z'$}\\
\frac{ \alpha' \beta'_{new}}{n'_{j..}+\alpha'} \hfill \text{New $z'$}\\
 \end{cases}
\end{equation*}

$p(z_{ji} = z| {\bf z_{-ji}}, z'_{ji} = z' )$ follows from Eqn. \ref{inference_zji_a}.

%\vspace*{0.1in} \noindent
{\bf Sampling $\beta$ and $\beta'$: }
The posterior of $G_0$, conditioned on samples $\psi_{k't}$ from it, is also distributed as a DP due to Dirichlet-Multinomial conjugacy, and the stick breaking weights of $G_0$ can be sampled as follows:
%\begin{equation*}
%\label{inference_beta}
$(\beta_1, \beta_2 \hdots \beta_K, \beta_{new} ) \sim Dir(m_{.1}, m_{.2} \hdots m_{.K}, \gamma)$
%\end{equation*}
Similarly, the stick breaking weights $\beta'$ can be sampled from the posterior distribution of $G'_0$ conditioned on samples from $G'_0$ in
the form of {$m'_{jk'}$} as follows:
%\begin{equation*}
%\label{inference_beta'}
$(\beta'_1, \beta'_2 \hdots \beta'_K, \beta'_{new} ) \sim Dir(m'_{.1}, m'_{.2} \hdots m'_{.K'}, \gamma')$
%\end{equation*}

%\vspace*{0.1in} \noindent 
{\bf Sampling $m$ and $m'$: }
$m_{k'k}$ is the number of inner tables generated as $n_{k'.k}$ samples are drawn from $G_k'$ that correspond to a particular topic $k$. 
This is the number of partitions generated as samples are drawn from a Dirichlet Process with concentration parameter 
$\alpha \beta_k$ and are distributed according to a closed form expression \cite{antoniak:aos74}. 
However, we adapt an alternate method \cite{Fox:AOAS2011} for sampling $m_{k'k}$  by drawing a 
total of $n_{k'.k}$ samples with topic k, and incrementing the count $m_{k'k}$ whenever a new inner table 
is created with topic assignment k.
% with probability $\alpha \beta_k$, for the topic $k$ 
Similarly, $m'_{jk'}$ is sampled by drawing a total of $n'_{j.k'}$ samples with entity k' and incrementing 
the count $m'_{jk'}$ whenever a new outer table is created with entity assignment $k'$.
%with probability $\alpha' \beta'_{k'}$, for entity $k'$.

%\vspace*{0.1in}\noindent 
{\bf Sampling Concentration parameters: }
We place a vague gamma prior on the concentration parameters $\alpha$, $\gamma$, $\alpha'$, $\gamma'$ with hyper parameters 
$\alpha_a , \alpha_b , \gamma_a, \gamma_b, \alpha'_a, \alpha'_b, \gamma'_a,$ and $\gamma'_b$ respectively. 
We use Gibbs sampling 
scheme for sampling the concentration parameters using the technique outlined in HDP\cite{HDP}.

%\vspace*{0.1in}
%\noindent {\bf Inference for Partially Observed Authors: }
%To fill in...
We use the conditional distributions above to perform inference under three different settings.
In the {\bf no observed entities} setting, the conditional distributions above are repeatedly sampled from until convergence.
For initialization, we first initialize the topic variables $z_{ji}$ using an online scheme, and then initialize the entities $z'_{ji}$ using the topics.
In the {\bf completely observed entities} setting, the set of entities $A_j$ is given for every document $j$.
Since no other entities are deemed possible for document $j$, $p(z'_{ji} = z' | {\bf z'_{-ji}} ,  {\bf z_{-ji}}, z_{ji} = z,  {\bf m}, {\bf m'}, \beta, \beta', {\bf x})$ is set to $0$ for new entities and for all $z'\notin A_j$.
In the {\bf partially observed entities} setting, a partial list of known entities $A_d$ is available for document $j$, but other entities are also possible.
We perform an initialization step, similar to that in the completely observed setting, using the known entities $A_j$. 
No new authors are added in this initial step. 
During later iterations, we allow all assignments $z'_{ji}=z$: one of the known entities from $A_j$, entities of other documents $j'$, and new entities.
However, we introduce a bias towards the known authors $z'\in A_j$ using an additional small positive term to their probability mass.%, to ensure these authors do not vanish and always have a non-zero probability of being selected.


==> inference_multilevel1.tex <==

\section{Inference}
\label{sec:multi-inference}
We use Gibbs sampling for approximate inference as exact inference is intractable for this problem. 
The conditional distributions from the nCRF scheme lend themselves to an inference algorithm, 
where we sample at every level 
$l \in \{0, \hdots, L\}$, the table assignments for customers {$t^l_{ji}$}, and dish assignments for tables 
{$k^l_{rt}$} where $1 \leq t \leq T^l_{r}$ and
${r} \in \{1, \hdots, K^{l+1}\}$, 
%$r=k^{l+1}_{j,i}$ 
since $\hat{k}$ is a restaurant identifier at level $l$ and the number of restaurants in level $l$ is same 
as the number of dishes in level $l+1$. Note that for the outermost level L, $K^{L+1}=M$, i.e the number of restaurants 
is the number of observed groups in the outermost level. This could correspond to the number of documents in a document modeling setting.
 
The conditional posterior for Gibbs sampling for these variables can be derived from the nCRF conditionals.
However, in such an approach, unlike the inference for a single level HDP, a naive approach of sampling all the 
above indices is intractable leading to an exponential complexity at each level due 
to the tight coupling between the variables. In this section, we briefly describe 
such an nCRF inference technique by sampling all the variables involved in the nCRF formulation to illustrate the computational 
intractability that arises, following which we describe an alternate scheme based on the 
direct sampling technique of HDP that overcomes this problem.

In this section, we discuss both these inference schemes, with a brief description of the naive nCRF scheme to illustrate 
its exponential complexity and then discuss the second scheme, i.e. the direct sampling scheme that we use in our experiments 
in \ref{experiments} for entity-topic analysis in more detail.
However in the appendix \ref{singledocInf}, we also discuss the first scheme, the naive nCRF inference algorithm in detail 
for a special case of the two-level nHDP using which we also experimentally demonstrate the difference in complexity between the 
two schemes.

\subsection{Inference Scheme 1: nCRF Inference}
\label{sec: ncrf}
In the basic nCRF scheme, the latent variables to be sampled as a part of the Gibbs sampling procedure are the assignment of 
tables to each customer $i$ belong to the observed group $j$ and dishes to tables at different levels. 
Hence, We wish to sample  $\forall l, $ {$t^l_{ji}$}, 
and {$k^l_{rt}$} where $r \in \{1, \hdots, K^{l+1}\}$ is a restaurant index at level $l$ also corresponding to 
a dish in level $l+1$ and $t \in \{1, \hdots, T^l_{r}\}$ is a table index in restaurant $r$. 
We start by sampling variables in level 0, the deepest level, proceeding to variables in level $L$. 
We attempt to illustrate in this section, how the complexity of 
sampling increases, reaching exponential complexity, as we go from sampling variables in level 0 through level L. 



We introduce the following notation for the rest of this section. We denote the set of all observed data as 
${\bf x}=\{x_{ji} : \forall j, i\}$.We denote the set of all customers going to table 
t of restaurant $r$ in level l as ${\bf x^l_{\hat{k}t}}=\{ x_{ji} : z^{l+1}_{ji}=\hat{k}, t^l_{ji}=t\}$. Further, a set with a subscript 
starting with a hyphen(-) indicates the set of all elements except the index following the hyphen. 

% Let $\textbf{x} = (x_{ji} :$ all $j,i),$ 
% ${\bf x_{-ji}} = (x_{j'i'} : j' \neq j , i' \neq i),$
% $\textbf{m} = (m^l_{k'k} :$ all $k',k,l),$  
% $\textbf{z} = (z^l_{ji} :$ all $j,i,l),$ 
% ${\bf z^l_{-ji}} = (z^{l'}_{j'i'} : j' \neq j , i' \neq i, l' \neq l),$
% and $\beta^l_{new}= \sum_{k=K^l+1}^{\infty} \beta^l_k$

We start with sampling of level 0 dish assignments to tables, conditioned on values of table and dish assignments at all 
other levels. Hence, we sample  $k^0_{\hat{k}t}$ as follows, for $\hat{k} \in \{1, \hdots, K^1\}$, $t \in \{ 1, \hdots, T^0_{\hat{k}}\}$ by
integrating out $G^0_0$ 
\begin{align}
\label{level0:ncrf}
p(k^0_{\hat{k}t} = k'| {\bf k^0_{-\hat{k},t}}, {\bf k^{-0}}, {\bf t}, {\bf x_{..}}) \propto \\ \nonumber
\begin{cases}
\frac{m^0_{k'}}{\gamma^0 + T^0_.}   p({\bf x^0_{\hat{k}t} } | k^0_{\hat{k}t} = k', {\bf k^0_{-\hat{k},t}}, {\bf k^{-0}}, {\bf t}) \hfill \text{where } k'\in\{1, \hdots, K^1\}\\
\frac{\gamma^0}{\gamma^0 + T^0_.}  p({\bf x^0_{\hat{k}t}}  | k^0_{\hat{k}t} = K^0+1, {\bf k^0_{-\hat{k},t}}, {\bf k^{-0}}, {\bf t})  \hfill \text{  new level 0 dish}
 \end{cases}
\end{align}
The first term is obtained from the conditional probability of the CRP for choosing level 0 dishes. 
We note that the likelihood terms  $p({\bf x^0_{\hat{k}t}}  | k^0_{\hat{k}t} = k', {\bf k^0_{-\hat{k},t}}, {\bf k^{-0}}, {\bf t})$  and  
$p({\bf x^0_{\hat{k}t}}  | k^0_{\hat{k}t} = K^0+1, {\bf k^0_{-\hat{k},t}}, {\bf k^{-0}}, {\bf t})$  arise from the probability of 
all observed data or customers that go to table $t$ of restaurant $r$ at level 0 that are affected by the assignment 
$k^0_{\hat{k}t} = k'$. These terms can be simplified by integrating out the appropriate $\phi$ variables corresponding to the topic 
multinomials. (A detailed evaluation for these terms is shown in appendix \ref{nCRFlikelihood}).
We further note that this update is similar to that in the direct sampling scheme for a single level HDP in  \cite{HDP}.
% 
% Next, the update for $t^0{ji}$ is obtained as follows for $\forall i,j$
% \begin{equation}
% p(t^0_{j,i} | t^0_{-ji}, k, X) \propto 
% \begin{Cases}
% \frac{m^0_{k'}}{\gamma^0 + T^0_.}  f_{k'} (x^0_{kt}) \hfill \text{where } k'=1, \hdots, K^0\\
% \frac{\gamma^0}{\gamma^0 + T^0_.}  f_{k'_{new}} (x^0_{kt})  \hfill \text{  new level 0 dish} 
% \end{Cases}
%\end{equation}


For the next level, we sample the update for dish assignment to tables belonging to level $1$ restaurants, $k^1_{\hat{k}t}$ for each 
$\hat{k} \in \{1, \hdots, K^2\}$, $t \in \{ 1, \hdots, T^1_{r} \}$. 
Let ${\bf S}^1_{\hat{k}t}={\{t^0_{ji}: t^1_{ji} = t, z^2_{ji} = \hat{k} \}}$, the set of level 0 table 
assignments corresponding to all  customers ${j,i}$ who have been assigned the table t in level 1 restaurant $\hat{k}$,
%(Also corresponding to a level 2 dish assignment of $\hat{k}$). 
% \begin{align}
% p(k^1_{\hat{k}t} = k'| k^1_{\hat{k},t}, k^{-1}, t^{-0}, X) \propto \\ \nonumber
% \begin{cases}
% \frac{m^1_{k'}}{\gamma^1 + T^1_.}  p(x^1_{\hat{k}t}  | k^1_{\hat{k}t} = k', k^1_{-\hat{k},t}, k^{-1}, t^{-0} , t^0_{\{ji: t^1_{ji} \neq t|| Z^2_{ji} \neq k \}}) \hfill \text{where } k'=1, \hdots, K^1\\
% \frac{\gamma^0}{\gamma^0 + T^0_.}  p(x^1_{\hat{k}t} | k^1_{\hat{k}t} = K^1+1, k^1_{-\hat{k},t}, k^{-1}, t^{-0}, t^0_{\{ji: t^1_{ji} \neq t || Z^2_{ji} \neq k \}})  \hfill \text{  new level 1 dish}
%  \end{cases}
% \end{align}
\begin{align}
p(k^1_{\hat{k}t} = k'| {\bf k^1_{-\hat{k},t}}, {\bf k^{-1}}, {\bf t^{-0}}, {\bf x}) \propto \\ \nonumber
\begin{cases}
\frac{m^1_{k'}}{\gamma^1 + T^1_.}  p({\bf x^1_{\hat{k}t}}  | k^1_{\hat{k}t} = k', k^1_{-\hat{k},t}, k^{-1}, \{{\bf t}-{\bf S}^1_{\hat{k}t} \}) \hfill \text{where } k'=1, \hdots, K^1\\
\frac{\gamma^0}{\gamma^0 + T^0_.}  p({\bf x^1_{\hat{k}t}} | k^1_{\hat{k}t} = K^1+1, {\bf k^1_{-\hat{k},t}}, {\bf k^{-1}}, \{{\bf t}-{\bf S}^1_{\hat{k}t} \})  \hfill \text{  new level 1 dish}
 \end{cases}
\end{align}
We note that the likelihood terms are conditioned on all table assignments 
except those in the set ${\bf S}^1_{\hat{k}t}$ since changing the level 1 dish assignment $k^1_{\hat{k}t}$ of 
the table in restaurant $\hat{k}$ changes the level 0 restaurant that the customer enters, due to which table assignments
in set ${\bf S}^1_{\hat{k}t}$ are not known.

Hence, evaluating the likelihood term requires marginalizing over all possible 
assignments for latent variables ${\bf S}^1_{\hat{k}t}$. We note that each of these variables can take a value 
between $1, \hdots, T^0_{k'}+1$. This leads to $(T^0_{k'}+1)^{|{\bf S}^1_{\hat{k}t}|}$ operations to simplify the likelihood term 
leading to an exponential complexity for evaluating the update $k^1_{kt}$ rendering this inference technique intractable.

We see that similarly, for a general level $l$, sampling $k^l_{\hat{k}t}$ for $k= \in \{1, \hdots, K^{l+1}\}$, 
$t \in \{ 1, \hdots, T^0_{\hat{k}}\} $ 
requires the marginalization over the following set ${\bf S}^l_{\hat{k}t}$ of all table assignments in all previous levels $\hat l < l$ 
for the customers sitting at the particular table $t$ in level $l$ restaurant $r$ :
$${\bf S}^l_{\hat{k}t}={\{t^{\hat l}_{ji}: \hat l<l, t^l_{ji} = t, z^{l+1}_{ji} = \hat{k} \}}$$
We see that the cardinality of this set increases exponentially with increasing $l$ due to which this technique is intractable for a general $l$, 
the only exception being $l=0$ for a single level HDP where this technique is tractable as in equation \ref{level0:ncrf}.

\subsection{Inference Scheme 2: Direct Sampling Scheme}
\label{sec: direct}
To work around the exponential complexity encountered in the previous section, we adopt a technique similar to the 
direct sampling scheme in \cite{HDP} where the variables   {$t^l_{ji}$}, and {$k^l_{rt}, \forall l,j,i,r,t$}
are not explicitly sampled. Instead the variables $G^l_0$ are explicitly sampled for all levels $l$ as opposed to being 
integrated out, by sampling the stick breaking weights $\beta^l$  respectively. Further, 
we directly sample {$z^l_{ji}$}, the \emph{dish assignment} at level $l$ for each customer(word) $i$, in each group(document) $j$, 
avoiding explicit assignments of tables to customers and dishes to tables. 
However, in order to sample $\beta^l$, the table information is maintained in the form of the aggregated 
counts in each layer, {$m^l_{r k}$}, the number of tables at level $l$, in restaurant $ r \in \{1, \hdots, K^{l+1}\}$ 
assigned to dish  $k \in \{1, \hdots, K^{l}\}$. (Recall that each restaurant at level $l$ corresponds to a unique dish 
in level $l+1$. Hence, $ r \in \{1, \hdots, K^{l+1}\}$. )
Thus the latent variables that need to be sampled in the Gibbs sampling 
scheme are {$z^l_{ji}$},  $\beta^l$, {$m^l_{r k}$}, $\forall l,i,j, r, k$.

We introduce the following notation for the rest of this section. 
Let $\textbf{x} = (x_{ji} :$ all $j,i),$ 
${\bf x_{-ji}} = (x_{j'i'} : j' \neq j , i' \neq i),$
$\textbf{m} = (m^l_{r k} :$ all $r,k,l),$  
$\textbf{z} = (z^l_{ji} :$ all $j,i,l),$ 
${\bf z^l_{-ji}} = (z^{l'}_{j'i'} : j' \neq j , i' \neq i, l' \neq l),$
and $\beta^l_{new}= \sum_{k=K^l+1}^{\infty} \beta^l_k$
We now provide the sampling updates for dish assignments for customers at each level, starting from level $0$, 
conditioned on all other dish assignments at all levels. 

%\vspace*{0.1in} \noindent
{\bf Sampling {$z^0_{ji}$}: } The conditional distribution for the dish assignment at level 0,  $z^0_{ji}$, depends on the 
predictive distribution of the dish assignment $z^0_{ji}$, given all other dish assignment to customers at this level 
and all other levels and the emission probabilities of the final observed data $x_{ji}$ with the specific dish assignment. 
This is given by
\begin{equation*}
%\label{inference_zji}
\begin{split}
 p(z^0_{ji} = p |z^1_{ji}=r , {\bf z^0_{-ji}},  {\bf m}, \beta, {\bf x}) 
 \propto p(z^0_{ji} = p| {\bf z^0_{-ji}}, z^1_{ji}=r ) p(x_{ji} | z^0_{ji} = p, {\bf x_{-ji}}) 
 \end{split}
\end{equation*}

To pick dish $p$ at level 0, conditioned on the dish assignment at level 1 as $r$, the first term 
$p(z^0_{ji} = p| {\bf z^0_{-ji}}, z^1_{ji}=r )$ can be split into two parts. One for 
 picking any of the existing tables from the level 0 restaurant $r$ that get mapped to dish $p$ 
 and one from creating a new table in restaurant $r$ and assigning dish $p$ to it. 
In the instance of  choosing a new dish, a new table is always created in restaurant $r$ at level 0. Hence,
 \begin{equation}
\label{inference_zji_a}
 p(z^0_{ji} = p| z^1_{ji}=r, {\bf z^0_{-ji}} ) \propto 
 \begin{cases}
\frac{n^0_{r.p} + \alpha \beta^0_p}{n_{r,.}+\alpha^0}   \hfill \text{  Existing dish}\\
\frac{\alpha^0 \beta^0_{new}}{n^0_{r.}+\alpha^0}   \hfill \text{  New dish}
 \end{cases}
\end{equation}

The likelihood term $p(x_{ji} | z_{ji} = z, {\bf x_{-ji}}) $ is the conditional density of $x_{ji}$ under 0 level dish(topic) $z^0_{ji}$  given all data items except $x_{ji}$. 
Assuming the 0 level dish is a topic sampled from a V dimensional symmetric Dirichlet prior over the vocabulary 
with parameter $\eta$, i.e $\phi_k \sim Dir(\eta)$, the conditional can be simplified to the following expression, 
by integrating out $\phi$.
 \begin{equation*}
%\label{inference_zji_b}
 p(x_{ji} = w | z^0_{ji} = p, {\bf x_{-ji}})  \propto \frac{ n^0_{pw} + \eta}{n^0_p. +  V \eta}
\end{equation*}
where $n^0_{pw}$ is the number of occurrences of level 0 dish(topic) p with word w in the vocabulary.
We note that this step is similar to that in \cite{HDP}.


%\vspace*{0.1in}\noindent
{\bf For any general level, sampling {$z^l_{ji}$}: } The conditional distribution for the dish assignment at level $l$ 
is computed as  
\begin{equation*}
%\label{inference_z'ji}
\begin{split}
 p(z^l_{ji} = p | {\bf z^l_{-ji}}, z^{l+1}_{ji}=r, z^{l-1}_{ji}=q, {\bf z^l_{-ji}} ,  {\bf m}, \beta,  {\bf x})  \\
 \propto p(z^l_{ji} = p| {\bf z^l_{-ji}}, z^{l+1}_{ji} = r) p(z^{l-1}_{ji} = q| {\bf z^{l-1}_{-ji}}, z^l_{ji} = p )
 \end{split}
\end{equation*}

 The first term is the predictive distribution of $z^l_{ji}$ given the next level dish assignment $r$ (to specify
 which level $l$ restaurant the customer goes to), while the second term arises from the previous level dish 
 assignment $q$ that depends on the value of $z^l_{ji}$. Again, $p(z^l_{ji} = p| {\bf z^l_{-ji}}, z^{l+1}_{ji} = r)$ can be viewed as consisting of two terms. One from 
 picking an existing table in restaurant $r$ with dish assignment $p$ and one from creating a new table 
 in restaurant $r$ at level $l$ and assigning the dish $p$ to it. 
 Further, creation of a new dish always involves the creation of a new table. Hence, 
 \begin{equation*}
%\label{inference_z'ji_a}
 p(z^l_{ji} = p | {\bf z^l_{-ji}}, z^{l+1}_{ji} = r ) \propto 
 \begin{cases}
\frac{n^l_{rp} + \alpha^l \beta^l_{p}}{n^l_{r.}+\alpha^l} \hfill \text{Existing dish}\\
\frac{ \alpha^l \beta^l_{new}}{n^l_{r.}+\alpha^l} \hfill \text{New dish}\\
 \end{cases}
\end{equation*}

Similarly 
\begin{equation*}
%\label{inference_z'ji_a}
 p(z^{l-1}_{ji} = q | {\bf z^{l-1}_{-ji}}, z^{l}_{ji} = p ) \propto 
 \begin{cases}
\frac{n^{l-1}_{pq} + \alpha^{l-1} \beta^{l-1}_{q}}{n^{l-1}_{p.}+\alpha^{l-1}} \hfill \text{Existing dish}\\
\frac{ \alpha^{l-1} \beta^{l-1}_{new}}{n^{l-1}_{p.}+\alpha^{l-1}} \hfill \text{New dish}\\
 \end{cases}
\end{equation*}

%$p(z_{ji} = z| {\bf z_{-ji}}, z'_{ji} = z' )$ follows from Eqn. \ref{inference_zji_a}.

%\vspace*{0.1in} \noindent
{\bf Sampling $\beta$ : }
At each level $l$, the posterior of $G^l_0$, conditioned on samples observed from it, is also distributed as a DP due 
to Dirichlet-Multinomial conjugacy, and the stick breaking weights of $G^l_0$ can be sampled as follows:
%\begin{equation*}
%\label{inference_beta}
$$(\beta^l_1, \beta^l_2 \hdots \beta^l_{K^l}, \beta_{new} ) \sim Dir(m^l_{.1}, m^l_{.2} \hdots m^l_{.K}, \gamma^l)$$
%\end{equation*}

%\vspace*{0.1in} \noindent 
{\bf Sampling $m$ : }
$m^l_{r k}$ is the number of tables in level $l$ restaurant $r \in \{1, \hdots, K^{l+1}\}$ 
%(also corresponding to a dish in level $l+1$)
 that are assigned to the level $l$ dish $k \in \{1, \hdots, K^{l}\}$.
%where $K^{L+1}=M$ 
%This is equivalent to the the number of new tables generated in restaurant $r$ while simulating a CRF  where
In other words, $m^l_{r k}$ is the number of tables created as  $n^l_{r.k}$ samples are drawn from $G^l_{r}$ in restaurant $r$ that correspond to a particular dish $k$. 
This is the number of partitions generated as samples are drawn from a Dirichlet Process with concentration parameter 
$\alpha^l \beta^l_k$ and are distributed according to a closed form expression \cite{antoniak:aos74}. 
However, we adapt an alternate method \cite{Fox:AOAS2011} for sampling $m^l_{rk}$  by drawing a 
total of $n^l_{r.k}$ samples with dish k, and incrementing the count $m^l_{r k}$ whenever a new table is created 
in restaurant $r$ with dish assignment k.
% with probability $\alpha \beta_k$, for the topic $k$ 
%with probability $\alpha' \beta'_{k'}$, for entity $k'$.

%\vspace*{0.1in}\noindent 
{\bf Sampling Concentration parameters: }
We place a vague gamma prior on the concentration parameters $\alpha^l$, $\gamma^l$ $\forall l$ with hyper parameters 
$\alpha_a , \alpha_b , \gamma_a, \gamma_b$ respectively. 
We use Gibbs sampling scheme for sampling the concentration parameters using the technique outlined in \cite{HDP}.

\section{Experimental evaluation of inference complexity}
%In this section we briefly discuss the inference complexity of the two proposed inference schemes, the nCRF scheme and the 
%direct sampling scheme. 

The nCRF scheme (Scheme 1) is computationally more expensive than the direct sampling scheme.
Scheme 1, as described in section \ref{sec: ncrf}, runs to exponential complexity even for the 2 level 
nHDP. Hence, we introduced the direct sampling scheme in section \ref{sec: direct} to outline a tractable inference algorithm. 
In this section, we illustrate this through some examples.

First we perform experiments with the single level nHDP, to compare the inference (training time) 
with both these schemes. The results of this experiment is shown in figure \ref{L1:compare_runtime}.
We also compare the perplexity obtained on held out test data with both these schemes for the single level nHDP. 
The perplexity results on the NIPS dataset with 20 percent of the documents held out is shown in 
table \ref{L1perplexity}. We note that while the nCRF scheme (scheme 1) performs better in terms of perplexity,
the direct sampling scheme is faster. This difference in complexity increases exponentially as we add more levels 
to the nHDP.

To better illustrate the difference in computational complexity between the two schemes, in this section, 
we compare the runtime of these two algorithms for a special case of our 2-level nHDP model where there is a single 
restaurant in the outer most level. In this special setting, at the outer most level, the HDP can be replaced by a simple DP since 
there is no sharing of atoms required between restaurants.
We discuss both the naive nCRF and the direct sampling inference algorithm for this setting in detail in appendix \ref{singledocInf}.
We perform experiments on a 100 document subset of the NIPS dataset to compare runtime in this 
special setting. The results are shown in figure \ref{compare_runtime}.
We note that the direct sampling technique is order of magnitude faster with respect to runtime complexity as 
illustrated in the figures \ref{compare_runtime}.
%and \ref{compare_likelihood}.
\begin{figure*}[!Htbp]
\begin{subfigure}{.48\textwidth}
\centering
\includegraphics[height=2.5in,width=2.5in]{L1_timecomp.eps}
\caption{\small \sl Comparison of runtime of Direct Sampling vs nCRF : We see that direct sampling runs for several iterations 
before the nCRF technique completes the first few Gibbs sampling iterations}  
\label{L1:compare_runtime}
\end{subfigure}
\begin{subfigure}{.04\textwidth}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
%\end{figure*}  
%\begin{figure*}[!Htbp]
\centering
\includegraphics[height=2.5in,width=2.5in]{timing_plot_comparison.eps}
\caption{\small \sl Comparison of runtime of Direct Sampling vs nCRF for single level HDP }  
\label{compare_runtime}
\end{subfigure}
\end{figure*}  
% \begin{figure*}[!Htbp]
% \centering
% \includegraphics[height=1.5in,width=5.7in]{direct_vs_ncrf_compare_fullrunto_2Kand500.eps}
% \caption{\small \sl Comparison of training likelihood of the nCRF vs Direct sampling scheme. 
% The nCRF scheme seems to be converging to a higher likelihood solution quickly due to faster mixing 
% compared to the direct sampling scheme. }  
% \label{compare_likelihood}
% \end{figure*}  
\begin{table}[t]
\centering
%\begin{tabular}{|l|c|}
%\hline
%Model& Perplexity\\
%\hline
%\hline
%ATM & 2783\\
%\hline
%HDP & 1775\\
%\hline
%nHDP\-co & 1247 \\
%\hline
%\end{tabular}
\begin{tabular}{|l|c|c|}
\hline
Model & Direct Sampling & nCRF \\
\hline
\hline
Perplexity & 2230 & 1937 \\
\hline
\end{tabular}
\caption{Perplexity comparison for single level nHDP for NIPS dataset with different inference schemes}\label{tab:L1co}
\label{L1perplexity}
\end{table}


==> infmixture1.tex <==
\subsection{ nHDP as Infinite Limit of a collection of Finate Mixture Models:}

A Dirichlet process mixture model can be derived as the infinite limit of a finate mixture model as the number of mixture componants 
tends to infinity[Eshwaran and Zaphaeur]. In \cite{HDP}, the authors have shown a similar result where 
a HDP can be constructed as an infinite limit of a collection of finate mixture models. We show a similar result for nHDP. 

We first define the following collection of finite mixtures. Consider a multi-level setting, 
with $l\in{0, \hdots,L}$ denoting the level, where each level has multiple group level distributions 
$G^l_{\hat k|K^l}$, $\hat k\in\{1,\hdots,K^{l+1}\}$ and a base level distribution $G^l_{0|K^l}$.  
Note that we use the notation $G^l_{\hat k|K^l}$ to denote that the distribution $G^l_{\hat k}$ has a finite number ($K^l$) of atoms.
%Let $K^l$ is the finite number of atoms corresonding to each group level distribution in level l, 
%and where each level $l\in{0, \hdots,L}$ has $K^{l+1}$ groups each corresponding
Further, these group level distributions at each level $l$ form the atoms of the next level $l+1$ defining 
a collection of finite mixtures as follows. 
%to the atoms of the next level $l+1$ and for the outermost group $K^{L+1}=M$ : 
\begin{gather*}
 \beta^0 | \gamma^0 \sim Dir (\frac{\gamma^0}{K^0}, \hdots , \frac	{\gamma^0}{K^0})  \tab \text{and} 
 \tab G^0_{0|K^0}= \sum_{k=1}^{K^0} \beta^0_k \delta{\phi_k} \\
 \forall \hat k \in \{1,\hdots, K^1\}, \text{ } \pi^0_{\hat k} | \alpha^0 \sim Dir(\alpha^0 \beta^0) \tab \text{and} \tab G^0_{\hat k|K^0}=\sum_{k=1}^{K^0} \pi_{\hat kk} \delta{\phi_k} \\
\text{For each level $l \in \{1,\hdots, L-1\}$,}\\
\beta^l | \gamma^l \sim Dir (\frac{\gamma^l}{K^l}, \hdots , \frac{\gamma^l}{K^l}) \tab \text{and} \tab G^l_{0|K^l}= \sum_{k=1}^{K^l} \beta^l_{k} \delta_{G^{l-1}_{k}}  \\
\forall \hat k \in \{1,\hdots, K^{l+1}\}, \text{ } \pi^l_{\hat k} | \alpha^l \sim Dir(\alpha^l \beta^l)  \tab \text{and} \tab G^l_{\hat k|K^l}=\sum_{k=1}^{K^l} \pi^l_{\hat kk} \delta_{G^{l-1}_{k}} \\
%\text{For the outermost level $L$, with M groups, }\\
%\beta^L | \gamma^L \sim Dir (\frac{\gamma^L}{K^L}, \hdots , \frac{\gamma^L}{K^L}) \tab \text{and} \tab G^L_{0|K^L}= \sum_{k=1}^{K^L} \beta^L_{k} \delta_{G^{L-1}_{k}}  \\
%\forall j \in \{1,\hdots, M\}, \text{ } \pi^L_{j} | \alpha^L \sim Dir(\alpha^L \beta^L)  \tab \text{and} \tab G^L_{j|K^L}=\sum_{k=1}^{K^L} \pi^l_{jk} \delta_{G^{L-1}_{k}} 
\end{gather*}

{\bf Theorem:} For each $l \in \{0,\hdots, L\}$,  with $G^l_{0|K^l}$ and $G^l_{\hat k|K^l}$ defined as above, 
as $K^l \to \infty, \forall l \in \{0,\hdots, L\}$, $G^l_{0|K^l} \to G^l_0$ (with $G^l_0$ as defined in section \ref{sec:multilevel}), 
and $\forall \hat k \in \{1,\hdots, K^{l+1}\}$, $G^l_{\hat k|K^l} \sim DP(\alpha^l, G^l_0)$ 

{\bf Proof:} We note that as $K^0 \to \infty$, $G^0_{0|K^0} \to G^0_0$ where the convergence of measures is defined by 
$\int g dG^0_{0|K^0} \xrightarrow[]{D} \int g dG^0_0$ for all real valued functions $g$ measurable with respect to $G^0_0$ as shown by 
[Ishwaran and Zarepour, 2002].  We note that we already have $G^0_{\hat k|K^0} \sim DP(\alpha^0, G^0_{0|K^0})$. 
This follows from the definition of the DP since $G^0_{\hat k|K^0}$ follows equation \ref{eqn:dp} with respect to the 
base measure $ G^0_{0|K^0}$ and the concentration parameter $\alpha^0$.
%for for every finite measurable partitioning $\{A_1, \hdots , A_F\}$ of $\Theta$,  one can show $(G^K_{\hat k}(A_1), \hdots, G^K_{\hat k}(A_F)) \sim Dir(\alpha G^K_0(A_1), \hdots, 
%\alpha G^K_0(A_n)$ from the properties of Dirichlet distribution. 
As $K^0 \to \infty$, we have already established that $G^0_{0|K^0} \to G^0_0$. Hence it follows that 
$G^0_{\hat k|K^0} \sim DP(\alpha^0, G^0_0)$ as $K^0 \to \infty$. 
for each level  $l \in \{1,\hdots, L\}$, having proved this result for all previous levels, assuming 
$K^{l'}\to \infty, \forall l'<l$, we can make a similar argument for level $l$ as that for level 0 
to conclude 
$G^l_{0|K^l} \to G^l_0$, and $\forall \hat k \in \{1,\hdots, K^{l+1}\}$, $G^l_{\hat k|K^L} \sim DP(\alpha^l, G^l_0)$.
This concludes the proof.


{\bf Alternate construction based on the nCRF}: The following alternate construction based on the nCRF, is another way to show nHDP as an infinite limit of a 
collection of finite mixture models, similar to that in \cite{HDP}, using the table and the dish indices of nCRF from 
the restaurant analogy as follows. 
\begin{gather*} \text{For level $l\in\{1,\hdots,L\}$, } \tab \beta^l | \gamma^l \sim Dir (\frac{\gamma^l}{K^l}, \hdots , \frac{\gamma^l}{K^l}) \\
\forall \hat k \in \{1,\hdots, K^l\},  \pi^l_{\hat k} | \alpha^l \sim Dir(\frac{\alpha^l}{T^l_{\hat k}}, \hdots, \frac{\alpha}{T^l_{\hat k}}) 
\tab k^l_{\hat kt} | \beta^l \sim \beta^l \tab \forall t\in\{1,\hdots,T^l_{\hat k}\}  
\end{gather*}
%t_{ji:Z'_{ji}=\hat k} | \pi_{\hat k} \sim \pi_{\hat k} 
In level L, for each outermost group $j\in\{1,\hdots,M\}$, for each observation, $i\in\{1,\hdots,N_j\}$,\\
\begin{gather}
\label{nCRF_finite}
t^L_{ji} | \pi^L_{j} \sim \pi^L_{j} \tab \text{and} \tab  z^L_{ji}=k^L_{jt^L_{ji}}  \\ \nonumber
% 
% \[ \beta' | \gamma' \sim Dir (\frac{\gamma'}{A}, \hdots , \frac{\gamma'}{A}) \tab  \hat k_{jt'} | \beta' \sim \beta'\]
% \[ \pi'_{j} | \alpha \sim Dir(\frac{\alpha'}{T'_{j}}, \hdots, \frac{\alpha'}{T'_{j}}) \tab  t'_{ji} | \pi'_{j} \sim \pi'_{j}\]
\text{For each level, $l\in\{L-1,\hdots,0\}$ } \tab  t^l_{ji} | z^{l+1}_{ji}=k, \pi^l_{k} \sim \pi^l_{k} \tab \text{and} \tab  z^l_{ji}=k^l_{z^{l+1}_{ji}t^l_{ji}} \\ \nonumber
 %\[\forall j, \forall i   \]
\text{And finally, } \tab x_{ji} | z^0_{ji}, \phi \sim \phi_{z^0_{ji}} 
\end{gather}
% 
% \[ \beta | \gamma \sim Dir (\frac{\gamma}{K}, \hdots , \frac{\gamma}{K}) \tab k_{\hat kt} | \beta \sim \beta \]
% \[ \pi_{\hat k} | \alpha \sim Dir(\frac{\alpha}{T_{\hat k}}, \hdots, \frac{\alpha}{T_{\hat k}}) \tab t_{ji:Z'_{ji}=\hat k} | \pi_{\hat k} \sim \pi_{\hat k}  \]
% 
% \[ \beta' | \gamma' \sim Dir (\frac{\gamma'}{A}, \hdots , \frac{\gamma'}{A}) \tab  \hat k_{jt'} | \beta' \sim \beta'\]
% \[ \pi'_{j} | \alpha \sim Dir(\frac{\alpha'}{T'_{j}}, \hdots, \frac{\alpha'}{T'_{j}}) \tab  t'_{ji} | \pi'_{j} \sim \pi'_{j}\]
% \[\forall j, \forall i \tab  Z_{ji}=k_{\hat k_{jt'_{ji}}t_{ji}} \]
%  \[\forall j, \forall i \tab  x_{ji} | Z_{ji}, \phi \sim \phi_{Z_{ji}} \]
% 
{\bf Theorem:} For each $l \in \{0,\hdots, L\}$,  
As $K^l \to \infty, \text{ and } T^l_{\hat k} \to \infty, \forall \hat k\in \{1,\hdots, K^{l+1}\}$,
the generative process described above in equation \ref{nCRF_finite} is equivalent to the nHDP.\\
{\bf Proof:} At each level $l$,  As $K^l \to \infty, \text{ and } T^l_{\hat k} \to \infty, \forall \hat k\in \{1,\hdots, K^{l+1}\}$,
%As $K \to \infty , T_{\hat k} \to \infty, A \to \infty $ and $T'_{j} \to \infty$, 
the predictive distribution of the draw from each Dirichlet distribution above tends to a CRP %\cite{CRP} 
and hence draws 
of $z^0_{ji}$ in the above construction in equation \ref{nCRF_finite} are the same as that from nCRF described in the previous section. 
Hence the collection of finite mixture models in \ref{nCRF_finite} tend to nHDP in the infinite limit.
%Hence we have constructed the nHDP as an infinite limit of a collection of finate mixture models.

%\subsection{ Stick breaking characterization of nHDP}
